Emotion and Theme Recognition in Music with Frequency-Aware RF-Regularized CNNs

We present CP-JKU submission to MediaEval 2019; a Receptive Field-(RF)-regularized and Frequency-Aware CNN approach for tagging music with emotion/mood labels. We perform an investigation regarding the impact of the RF of the CNNs on their performance on this dataset. We observe that ResNets with smaller receptive fields -- originally adapted for acoustic scene classification -- also perform well in the emotion tagging task. We improve the performance of such architectures using techniques such as Frequency Awareness and Shake-Shake regularization, which were used in previous work on general acoustic recognition tasks.

==> baselines.tex <==

\gerhard{Maybe this "Baselines" section should come *after* the Approach section? -- after all, the Approach is the main thing you want to present, and when you say "additional baselines" in the first sentence, then this must be in addition to something that has been presented before ...}

\verena{As additional baselines we trained a Resnet~\cite{heDeepResidualLearning2016} and a convolutional RNN (CRNN). The Resnet we used is a standard Resnet\footnote{\url{https://github.com/pytorch/vision/blob/master/torchvision/models/resnet.py}} with a minor modification in the first convolutional layer to work with spectrograms (1 channel) instead of RGB images (3 channels). In our preliminary experiments the Resnet-34 outperformed Resnet-18 and Resnet-50 on the validation set, so we picked this architecture as an additional baseline.} % more details on optimizer (Adam), and other things? (lr=0.0005, bs=16)

\shreyan{The CRNN network was motivated by the notion that global structure of musical features could affect the perception of certain aspects of music (like mood), as mentioned by Choi et al \cite{choi2017convolutional}. We use an architecture similar to the one used by Choi et al, where the CNN part acts as the feature extractor and the RNN part acts as a temporal aggregator. This approach increased the performance from the baseline CNN and the Resnet-34.}
